DES Y3 results: Blending shear and redshift biases in image simulations

As the statistical power of galaxy weak lensing reaches percent level precision, large, realistic and robust simulations are required to calibrate observational systematics, especially given the increased importance of object blending as survey depths increase. To capture the coupled effects of blending in both shear and photometric redshift calibration, we define the effective redshift distribution for lensing, $n_{\gamma}(z)$, and describe how to estimate it using image simulations. We use an extensive suite of tailored image simulations to characterize the performance of the shear estimation pipeline applied to the Dark Energy Survey (DES) Year 3 dataset. We describe the multi-band, multi-epoch simulations, and demonstrate their high level of realism through comparisons to the real DES data. We isolate the effects that generate shear calibration biases by running variations on our fiducial simulation, and find that blending-related effects are the dominant contribution to the mean multiplicative bias of approximately $-2\%$. By generating simulations with input shear signals that vary with redshift, we calibrate biases in our estimation of the effective redshfit distribution, and demonstrate the importance of this approach when blending is present. We provide corrected effective redshift distributions that incorporate statistical and systematic uncertainties, ready for use in DES Year 3 weak lensing analyses.

==> authorlist.tex <==
% Author list file generated with: mkauthlist 1.2.4+6.g9cbd239 
% mkauthlist -j mnras DES-2020-0550_author_list_ordered.csv 

\author[DES Collaboration]{
\parbox{\textwidth}{
\Large
N.~MacCrann,$^{1,\dag}$
M.~R.~Becker,$^{2}$
J.~McCullough,$^{3,5}$
A.~Amon,$^{3}$
D.~Gruen,$^{4,3,5}$
M.~Jarvis,$^{6}$
A.~Choi,$^{7}$
M.~A.~Troxel,$^{8}$
E.~Sheldon,$^{9}$
B.~Yanny,$^{10}$
K.~Herner,$^{10}$
S.~Dodelson,$^{11}$
J.~Zuntz,$^{12}$
K.~Eckert,$^{6}$
R.~P.~Rollins,$^{13}$
T.~N.~Varga,$^{14,15}$
G.~M.~Bernstein,$^{6}$
R.~A.~Gruendl,$^{16,17}$
I.~Harrison,$^{13,18}$
W.~G.~Hartley,$^{19}$
I.~Sevilla-Noarbe,$^{20}$
A.~Pieres,$^{21,22}$
S.~L.~Bridle,$^{13}$
J.~Myles,$^{4}$
A.~Alarcon,$^{2}$
S.~Everett,$^{23}$
C.~S{\'a}nchez,$^{6}$
E.~M.~Huff,$^{24}$
F.~Tarsitano,$^{25}$
M.~Gatti,$^{26}$
L.~F.~Secco,$^{6}$
T.~M.~C.~Abbott,$^{27}$
M.~Aguena,$^{28,21}$
S.~Allam,$^{10}$
J.~Annis,$^{10}$
D.~Bacon,$^{29}$
E.~Bertin,$^{30,31}$
D.~Brooks,$^{32}$
D.~L.~Burke,$^{3,5}$
A.~Carnero~Rosell,$^{33,34}$
M.~Carrasco~Kind,$^{16,17}$
J.~Carretero,$^{26}$
M.~Costanzi,$^{35,36}$
M.~Crocce,$^{37,38}$
M.~E.~S.~Pereira,$^{39}$
J.~De~Vicente,$^{20}$
S.~Desai,$^{40}$
H.~T.~Diehl,$^{10}$
J.~P.~Dietrich,$^{41}$
P.~Doel,$^{32}$
T.~F.~Eifler,$^{42,24}$
I.~Ferrero,$^{43}$
A.~Fert\'e,$^{24}$
B.~Flaugher,$^{10}$
P.~Fosalba,$^{37,38}$
J.~Frieman,$^{10,44}$
J.~Garc\'ia-Bellido,$^{45}$
E.~Gaztanaga,$^{37,38}$
D.~W.~Gerdes,$^{46,39}$
T.~Giannantonio,$^{47,48}$
J.~Gschwend,$^{21,22}$
G.~Gutierrez,$^{10}$
S.~R.~Hinton,$^{49}$
D.~L.~Hollowood,$^{23}$
K.~Honscheid,$^{7,50}$
D.~J.~James,$^{51}$
O.~Lahav,$^{32}$
M.~Lima,$^{28,21}$
M.~A.~G.~Maia,$^{21,22}$
M.~March,$^{6}$
J.~L.~Marshall,$^{52}$
P.~Martini,$^{7,53,54}$
P.~Melchior,$^{55}$
F.~Menanteau,$^{16,17}$
R.~Miquel,$^{56,26}$
J.~J.~Mohr,$^{41,14}$
R.~Morgan,$^{57}$
J.~Muir,$^{3}$
R.~L.~C.~Ogando,$^{21,22}$
A.~Palmese,$^{10,44}$
F.~Paz-Chinch\'{o}n,$^{47,17}$
A.~A.~Plazas,$^{55}$
M.~Rodriguez-Monroy,$^{20}$
A.~Roodman,$^{3,5}$
S.~Samuroff,$^{11}$
E.~Sanchez,$^{20}$
V.~Scarpine,$^{10}$
S.~Serrano,$^{37,38}$
M.~Smith,$^{58}$
M.~Soares-Santos,$^{39}$
E.~Suchyta,$^{59}$
M.~E.~C.~Swanson,$^{17}$
G.~Tarle,$^{39}$
D.~Thomas,$^{29}$
C.~To,$^{4,3,5}$
and R.D.~Wilkinson$^{60}$
\begin{center} (DES Collaboration) \end{center}
}
\vspace{0.4cm}
\\
\parbox{\textwidth}{
%\scriptsize
$^{1}$ Department of Applied Mathematics and Theoretical Physics, University of Cambridge, Cambridge CB3 0WA, UK\\
$^{2}$ Argonne National Laboratory, 9700 South Cass Avenue, Lemont, IL 60439, USA\\
$^{3}$ Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA\\
$^{4}$ Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA\\
$^{5}$ SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA\\
$^{6}$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA\\
$^{7}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{8}$ Department of Physics, Duke University Durham, NC 27708, USA\\
$^{9}$ Brookhaven National Laboratory, Bldg 510, Upton, NY 11973, USA\\
$^{10}$ Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA\\
$^{11}$ Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA\\
$^{12}$ Institute for Astronomy, University of Edinburgh, Edinburgh EH9 3HJ, UK\\
$^{13}$ Jodrell Bank Centre for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK\\
$^{14}$ Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany\\
$^{15}$ Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany\\
$^{16}$ Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA\\
$^{17}$ National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA\\
$^{18}$ Department of Physics, University of Oxford, Denys Wilkinson Building, Keble Road, Oxford OX1 3RH, UK\\
$^{19}$ D\'{e}partement de Physique Th\'{e}orique and Center for Astroparticle Physics, Universit\'{e} de Gen\`{e}ve, 24 quai Ernest Ansermet, CH-1211 Geneva, Switzerland\\
$^{20}$ Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain\\
$^{21}$ Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{22}$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{23}$ Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA\\
$^{24}$ Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA\\
$^{25}$ Department of Physics, ETH Zurich, Wolfgang-Pauli-Strasse 16, CH-8093 Zurich, Switzerland\\
$^{26}$ Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain\\
$^{27}$ Cerro Tololo Inter-American Observatory, NSF's National Optical-Infrared Astronomy Research Laboratory, Casilla 603, La Serena, Chile\\
$^{28}$ Departamento de F\'isica Matem\'atica, Instituto de F\'isica, Universidade de S\~ao Paulo, CP 66318, S\~ao Paulo, SP, 05314-970, Brazil\\
$^{29}$ Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\
$^{30}$ CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{31}$ Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{32}$ Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK\\
$^{33}$ Instituto de Astrofisica de Canarias, E-38205 La Laguna, Tenerife, Spain\\
$^{34}$ Universidad de La Laguna, Dpto. Astrofísica, E-38206 La Laguna, Tenerife, Spain\\
$^{35}$ INAF-Osservatorio Astronomico di Trieste, via G. B. Tiepolo 11, I-34143 Trieste, Italy\\
$^{36}$ Institute for Fundamental Physics of the Universe, Via Beirut 2, 34014 Trieste, Italy\\
$^{37}$ Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain\\
$^{38}$ Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain\\
$^{39}$ Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{40}$ Department of Physics, IIT Hyderabad, Kandi, Telangana 502285, India\\
$^{41}$ Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany\\
$^{42}$ Department of Astronomy/Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA\\
$^{43}$ Institute of Theoretical Astrophysics, University of Oslo. P.O. Box 1029 Blindern, NO-0315 Oslo, Norway\\
$^{44}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{45}$ Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain\\
$^{46}$ Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{47}$ Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{48}$ Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{49}$ School of Mathematics and Physics, University of Queensland,  Brisbane, QLD 4072, Australia\\
$^{50}$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{51}$ Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA\\
$^{52}$ George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA\\
$^{53}$ Department of Astronomy, The Ohio State University, Columbus, OH 43210, USA\\
$^{54}$ Radcliffe Institute for Advanced Study, Harvard University, Cambridge, MA 02138\\
$^{55}$ Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA\\
$^{56}$ Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain\\
$^{57}$ Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390\\
$^{58}$ School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK\\
$^{59}$ Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831\\
$^{60}$ Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK\\
}
}


